Over-the-Air Inference over Multi-hop MIMO Networks

A novel over-the-air machine learning framework over multi-hop multiple-input and multiple-output (MIMO) networks is proposed. The core idea is to imitate fully connected (FC) neural network layers using multiple MIMO channels by carefully designing the precoding matrices at the transmitting nodes. A neural network dubbed PrototypeNet is employed consisting of multiple FC layers, with the number of neurons of each layer equal to the number of antennas of the corresponding terminal. To achieve satisfactory performance, we train PrototypeNet based on a customized loss function consisting of classification error and the power of latent vectors to satisfy transmit power constraints, with noise injection during training. Precoding matrices for each hop are then obtained by solving an optimization problem. We also propose a multiple-block extension when the number of antennas is limited. Numerical results verify that the proposed over-the-air transmission scheme can achieve satisfactory classification accuracy under a power constraint. The results also show that higher classification accuracy can be achieved with an increasing number of hops at a modest signal-to-noise ratio (SNR).

==> SecI.tex <==
It has witnessed the trend of integrating computation and wireless communications to boost the future Internet of Things networks\cite{edge_comp_over, image_retrieval}. 
Instead of the traditional digital schemes where the computation and communication are separated, over-the-air computation (OAC)  enables integrated communication and computation using analog transmissions \cite{oac_fed, oac_amiri}. A key advantage of the OAC scheme is to shift the computation burden to the wireless domain by leveraging the inherent broadcast nature of
wireless signals. For instance, linear operations such as summations and polynomials can be carried out by signal-superposition properties which have been widely applied in the federated learning \cite{oac_fed, oac_amiri}. 

Although there are a large number of works focusing on federated learning based on the OAC, they failed to make full use of the MIMO  channels. The precoder was designed based on maximizing the communication utility, e.g., minimizing the computation minimum mean square of the (MSE) \textbf{\color{red}(provide references)}, 
 however, the ultimate goal of the task is to maximize the machine learning utility, e.g., maximizing the classification accuracy \textbf{\color{red}(provide references)}. To reach the ultimate machine learning goal, a concept of air fully-connected (FC) layer is proposed, where the effective wireless channel is treated as a prototype FC layer. The main idea is to customize the wireless channel by designing precoders or deploying reconfigurable intelligent surfaces. 

 motivation is unclear: 
 [1. list the existing works, and provide a brief discussion]; [2. conclude their drawback or something missing discussion,]; 




Despite the great success of introducing OAC to federate learning, the previous works failed to make full use of the wireless networks whose nodes are equipped with multiple antennas. Inspired by the similarity of the input-output relation between a MIMO channel with a precoding matrix and that of a fully connected (FC) layer, the authors in \cite{air_fc, air_mimo} developed multiple-input and multiple-output (MIMO)-based OAC schemes to implement efficient deep learning algorithms over the wireless networks. To be specific, in \cite{air_fc}, the authors constructed an FC layer using a multiple input single output (MISO) system. System-level validation was conducted and a high classification accuracy was achieved on the MNIST dataset. 
In \cite{air_mimo}, the authors studied a split learning framework where the FC layer is constructed using the precoding matrix at the transmitter, the combining matrix at the receiver, and the MIMO channel.  The gradients are back-propagated via the MIMO channel to update the precoding and combining matrices for each epoch. The concept is not limited to the MIMO system, the authors in \cite{air_ris} construct convolutional neural networks for modulation classification problem utilizing the wireless propagation principle of the reconfigurable intelligent surfaces.

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{./figures/system_model.pdf}\\
  \caption{The flowchart of the multi-hop MIMO network and the PrototypeNet. In particular, we consider the number of hop $N = 2$ for the wireless network which is equivalent to the PrototypeNet with two FC layers. The loss function to train the PrototypeNet is also shown in the figure.}
\label{fig:system_model}
\end{figure*}

In this paper, we consider over-the-air machine learning over multi-hop MIMO networks for image classification. Instead of the split learning over multiple base stations implemented in \cite{air_mimo} where each base station has abundant computation resources, in our scenario, each node only performs non-linear activation, power normalization and precoding. We notice that the multi-hop MIMO network resembles that of a complex-valued neural network with multiple FC layers which is dubbed as `PrototypeNet'. Thus, we first train the PrototypeNet to guide the design of the multi-hop MIMO network, especially the precoding matrices.
In particular, the PrototypeNet is trained in an end-to-end fashion using a loss function which is a combination of the classification error and the power of the latent vectors. The loss function is essential to achieve satisfactory classification performance under a power constraint.
Given the weights of the FC layers as well as the CSI for each hop, the precoding matrix is obtained by solving an optimization problem. This differs from that in \cite{air_mimo} where the precoding and combining matrices are trained along with the neural network weights at the base stations. 
We further consider extending the proposed scheme to the scenario where the nodes have limited number of antennas.
Numerical experiments are carried out to verify the effectiveness of the proposed scheme. We also show the relationship between the system performance and the number of hops where having more hops is beneficial with a modest SNR value.

==> SecII.tex <==
We consider image classification problem over multi-hop MIMO network where a source node ($\mathrm{S}$) delivers an image, denoted as ${\bf{S}} \in \mathbb{R}^{C\times H \times W}$, to the destination node, $\mathrm{D}$ with the aid of $(N-1)$ relay nodes, $\{\mathrm{R}_1, \ldots, \mathrm{R}_{N-1}\}$ where $C, H, W$ represent the number of channels, the height and the width of the image, respectively. Each image $\bm{S}$ belongs to a certain class, which can be represented via an one-hot vector $\bm{c} \in \mathbb{R}^K$ where $K$ is the total number of classes. The source, destination and the relay nodes are equipped with multiple antennas. We further assume that for each node, the CSI of its adjacent hops are available. The processing of each node is shown in the top of Fig. \ref{fig:system_model} and is detailed as follows.

To start with, the source node transforms the input image, $\bm{S}$ into a complex-valued vector, denoted as $\bm{s}_1^\prime \in \mathbb{C}^{M_1}$ via a function, $g(\cdot)$ which can be realized by 2d convolutional neural networks, 2d average pooling operation, e.t.c. Then, we apply power normalization (PN) to the complex vector $\bm{s}_1^\prime$ to obtain $\bm{s}_1$ which is expressed as:
\begin{equation}
    \bm{s}_1 = (\bm{s}_1^\prime - \mu_1)/v_1,
    \label{eq:s1}
\end{equation}
where $\mu_1$ and $v_1$ denote the moving mean and deviation of $\bm{s}_1^\prime$ which are recorded during training. The PN module ensures that $\mathbb{E}(||\bm{s}_1||^2_2) \le M_1$. The source node, $\mathrm{S}$ adopts a precoding matrix, $\bm{F}_1 \in \mathbb{C}^{M_1 \times M_1}$and the transmitted signal, denoted as $\bm{x}_1$ can be expressed as:
\begin{equation}
    \bm{x}_1 = \bm{F}_1 \bm{s}_1.
\end{equation}

After passing the channel, the received signal, $\bm{y}_1 \in \mathbb{C}^{M_2}$ at the first relay node, $\mathrm{R}_1$ can be expressed as:
\begin{align}
    \bm{y}_1 = \bm{H}_1 \bm{x}_1 + \bm{n}_1,
    \label{eq:mimo_channel}
\end{align}
where each element of $\bm{H}_1$ is independent and identically distributed (i.i.d.) following a complex Gaussian distribution, i.e., $\mathcal{CN}(0, 1)$ while the noise term, $\bm{n}_1 \sim \mathcal{CN}(\bm{0}, \sigma^2_1 \bm{I}_{M_2})$. 

At $\mathrm{R}_1$, the received signal $\bm{y}_1$ is first fed to the non-linear activation function, $\phi(\cdot)$ which is implemented as a complex ReLU function. To be precise, both the real and imaginary part of $\bm{y}_1$ are activated by the standard ReLU function. Power normalization is applied to the non-linear activation output to generate $\bm{s}_2$. We emphasize that the PN layer is essential to control the power transmitted over the relay nodes which facilitates the following descriptions.
The transmitted signal of the first relay node can be expressed as: 
\begin{align}
    {\bm{x}_2} = {\bm{F}_2}  {\rm PN}(\phi(\bm{y}_1)),
    \label{eq:operation_hops}
\end{align}
where $\bm{F}_2$ is the precoding matrix at $\mathrm{R}_1$ and ${\rm PN}$ denotes power normalization. We note that the remaining relay nodes follow the same procedure and we omit the detailed descriptions due to the page limit.

The received signal, $\bm{y}_N$ at the destination node is first fed into the complex ReLU function $\phi(\cdot)$ and is transformed into a real-valued $2M_N$-dimensional vector by concatenating the real and imaginary parts of the complex vector. After passing the FC layer, $f_c(\cdot)$, followed by the Softmax activation function, a probability vector, $\bm{p} \in \mathbb{R}^K$ is obtained and the index, $k^*$, of the largest element in $\bm{p}$ is the final classification output. The classification accuracy of the system is defined as:
\begin{align}
    \text{Acc} (\%) = \mathbb{E}(\bm{1}(k^* = c^*)),
    \label{eq:accuracy}
\end{align}
where $\bm{1}(\cdot)$ is the indicator function and $c^*$ denotes the correct index.
Note that we simplify the following discussion by assuming the number of antennas and the noise power are identical over the hops, i.e., $M_1 = \cdots = M_N \triangleq M$ and $\sigma_1^2 = \cdots = \sigma_N^2 \triangleq \sigma^2$. 

==> SecIII.tex <==
In this section, we first introduce the motivation and the training methodology of the PrototypeNet. Then, the procedure to obtain the precoding matrices, $\{\bm{F}_1, \cdots, \bm{F}_N\}$ are provided. 


\subsection{PrototypeNet}\label{sec:IIIA}
As illustrated in the introduction, for the $i$-th hop with MIMO channel realization, $\bm{H}_i$, we aim to determine a precoding matrix, $\bm{F}_i$ such that the received signal at the $(i+1)$-th node can be treated as the output of a FC layer (without the bias term). This is plausible as the received signal and the output of the $i$-th FC layer, $\bm{y}_{i+1}$ can be expressed as:
\begin{align}
    \bm{y}_{i+1} &= \bm{H}_i\bm{F}_i \bm{s}_i + \bm{n}_i, \\
    \bm{y}_{i+1} &= \bm{W}_i \bm{s}_i,
    \label{eq:Fi_vs_Wi}
\end{align}
where $\bm{W}_i$ represents the weight of the FC layer\footnote{The complex valued neural network is adopted which is available at: \url{https://github.com/wavefrontshaping/complexPyTorch}.}.
Thus, the problem can be formulated as finding $\bm{F}_i$ such that $\bm{H}_i\bm{F}_i$ is equivalent to $\bm{W}_i$. We will first introduce a novel end-to-end optimization algorithm to determine the weights, $\bm{W}_i$ which is detailed as follows.

To start with, we construct the PrototypeNet which resembles the wireless multi-hop network which is illustrated in Fig. \ref{fig:system_model}. In particular, both the PrototypeNet and the multi-hop MIMO network share the same transformation function, $g(\cdot)$, the PN modules and the FC layer, $f_c(\cdot)$.
At the first glance, the PrototypeNet is identical to the standard image classification network. However, we emphasize that the weights obtained by training a standard image classification network fails to achieve satisfactory performance when applied to the multi-hop MIMO network. This is due to the fact that the standard network does not take the Frobenius norms of $\bm{W}_i, i \in [1, N]$ (or equivalently, the power of $\bm{z}_i$) into account. Moreover, there is no channel noise introduced in the standard network leading to $\bm{W}_i, i \in [1, N]$ that are fragile to noise.
%In particular, each element of $\bm{W}_i$ can be scaled by an arbitrary factor without influencing the final reconstruction performance\footnote{This is because the PN module is capable to offset the effect of the scaling operations.}.  Though it is possible for the standard image classification network to control the power of the latents $\bm{z}_i$ by scaling the weights, $\bm{W}_i$, it would lead to sub-optimal performance as the latents may not be robust to noise. 
%Moreover, depending on different initialization, the weights, $\bm{W}_i$ obtained by the standard classification network can be quite different in terms of the frobneous norms. This leads to problems when deployed in the real wireless network due to the randomness of the weights, $\bm{W}_i$. 

To this end, the proposed PrototypeNet takes the power constraint as well as the channel noise into account. For the $i$-th node, after generating the complex vector $\bm{s}_i$ as in \eqref{eq:s1}, the neural network weight, $\bm{W}_i$ is multiplied with it and the noise, $\bm{n}_i$ is added to the output, $\bm{z}_i = \bm{W}_i \bm{s}_i$ to produce $\bm{y}_i$ for the next node:
\begin{align}
    \bm{y}_{i} = \bm{W}_i \bm{s}_i + \bm{n}_i.
    \label{eq:yi}
\end{align}
Intuitively, there exists a trade-off between the power of $\bm{z}_i$, $\|\bm{z}_i\|_2^2$ and the classification accuracy: when $\|\bm{z}_i\|_2^2$ is large, the noise $\bm{n}_i$ is neglectable and has little impact on the accuracy. On the other hand, when $\|\bm{z}_i\|_2^2$ is small, the noise dominates and the performance degrades significantly.

To achieve different trade-off points between the power and the accuracy, we consider two different loss functions to train the PrototypeNet as:
\begin{align}
    \mathcal{L}_1 &= -\sum_{k=1}^K c_k \log(p_k) +  \frac{\lambda}{N} \sum_{j=1}^N \|\bm{W}_j\|_F^2, \label{eq:optim_W} \\
    \mathcal{L}_2 &= -\sum_{k=1}^K c_k \log(p_k) +  \frac{\lambda}{N} \sum_{j=1}^N \|\bm{z}_j\|_2^2, \label{eq:optim_z}
\end{align}
where $\lambda$ balances the power and the classification accuracy for both schemes. Note that the second term of  $\mathcal{L}_1$, i.e., $\frac{\lambda}{N} \sum_{j=1}^N \|\bm{W}_j\|_2^2$ minimizes the Frobenius norm of the weights which is analogous to the widely used weight regularization terms to avoid over-fitting. In our case, this term implicitly minimizes the power of $\bm{z}_i$. The second loss function, $\mathcal{L}_2$ on the other hand, directly minimizes $\|\bm{z}_i\|_2^2$. We will show in the simulation part that training the PrototypeNet using $\mathcal{L}_2$ leads to more satisfactory results. Finally, we define the average received power, $P_{avg}^r$ over $N$ hops as:
\begin{align}
    P_{avg}^r = \frac{1}{N} \sum_{j=1}^N \|\bm{z}_j\|_2^2 = \frac{1}{N} \sum_{j=1}^N \|\bm{W}_j\bm{s}_j\|_2^2.
    \label{eq:P_avg_r}
\end{align}
Note that we are more interested in the average transmit power, $P^t_{avg}$ which is defined as:
\begin{equation}
    P^t_{avg} = \frac{1}{N} \sum_{i=1}^{N} \|\bm{F}_i \bm{s}_i\|_2^2,
    \label{eq:P_avg_t}
\end{equation}
However, since we have no access to $\bm{F}_i\bm{s}_i$ in the PrototypeNet, we use $P_{avg}^r$ as a substitution.


\begin{algorithm}[t!]
\caption{Optimization for the $i$-th precoding matrix, $\bm{F}_i$.}\label{alg:calculate_Fi}
\begin{algorithmic}[1]
\State{\textbf{Input} $\{\bm{W}_i, \bm{H}_i, \tilde{\mathcal{S}}_i, \lambda_1, \eta, \epsilon\}$; \textbf{Output} $\bm{F}_i$}
\State{\textbf{Initialize} $\bm{F}_i = \bm{H}_i^{-1} \bm{W}_i,$}
\State{\textbf{Objective} $G_{p} = \|\bm{W}_i - \bm{H}_i \bm{F}_i\|^2_F + \lambda_1 \text{tr}(\tilde{\mathcal{S}}_i\bm{F}_i^H\bm{F}_i)$}
\While{True}:

\State{\textbf{Calculate the gradient:} $\nabla \bm{F}_i = -2\bm{H}_i^H \bm{W}_i + 2\bm{H}_i^H \bm{H}_i \bm{F}_i + 2\lambda_1 \bm{F}_i \tilde{\mathcal{S}}_i$,}
\State{\textbf{Update:} $\bm{F}_i = \bm{F}_i - \eta \nabla \bm{F}_i$,}
\State{\textbf{New objective:} $G_c = \|\bm{W}_i - \bm{H}_i \bm{F}_i\|^2_F + \lambda_1 \text{tr}(\tilde{\mathcal{S}}_i\bm{F}_i^H\bm{F}_i)$,}
\If{$|G_c - G_p| < \epsilon$}
\State{\textbf{Return} $\bm{F}_i$.}
\Else
\State{$G_p = G_c$.}
\EndIf

\EndWhile
\end{algorithmic}
\end{algorithm}

\subsection{Calculation of $\bm{F}_i$}
After obtaining the weights $\bm{W}_i, i \in [1, N]$ from the PrototypeNet, we consider applying them to the multi-hop MIMO network. Take the first hop as an example, since $\bm{H}_1$ is available at the source node, the precoding matrix $\bm{F}_1$ will be determined using $\bm{W}_1$ and $\bm{H}_1$. 

Note that each element of $\bm{H}_1$ follows an i.i.d. complex Gaussian distribution, it can be shown that $\bm{H}_1$ is full-rank with probability equals to one. Thus, the inverse matrix of $\bm{H}_1$ always exists. A naive solution is to set 
\begin{equation}
    \bm{F}_1 = \bm{H}^{-\dagger}_1 \bm{W}_1,
    \label{eq:F_naive}
\end{equation}
such that $\bm{H}_1\bm{F}_1$ strictly equals to $\bm{W}_1$ and the corresponding classification accuracy is identical to that of the PrototypeNet. However, the naive approach leads to overwhelmingly high transmit power, $\|\bm{F}_1 \bm{s}_1\|^2_2$. This can be understood by the fact that the randomly generated $\bm{H}_1$ may be ill-conditioned and some singular values of $\bm{H}^{-\dagger}_1$ are extremely large. To this end, we propose an alternative approach to determine $\bm{F}_1$ which is detailed as follows.

We formulate an optimization problem with an objective to achieve a high classification accuracy while consuming low transmit power at the source node. For the former objective, since $\bm{W}_1$ has already been optimized, we expect the term $\|\bm{H}_1\bm{F}_1 - \bm{W}_1\|^2_F$ to be as small as possible. For the second one, we are interested in minimizing the expectation of the transmit power, i.e., $\mathbb{E}(\|\bm{F}_1 \bm{s}_1\|^2_2)$ over all $\bm{s}_1$. Note that $\mathbb{E}(\|\bm{F}_1 \bm{s}_1\|^2_2)$ can be alternatively expressed as:
\begin{equation}
    \mathbb{E}(\|\bm{F}_1 \bm{s}_1\|^2_2) = \mathbb{E}(\text{tr}(\bm{S}_1\bm{F}_1^H\bm{F}_1)) = \text{tr}(\mathcal{S}_1\bm{F}_1^H\bm{F}_1),
    \label{eq:power_expect}
\end{equation}
where $\bm{S}_1 =  \bm{s}_1\bm{s}_1^\dagger$, $\mathcal{S}_1 \triangleq \mathbb{E}(\bm{S}_1)$ and $\text{tr}(\cdot)$ calculates the trace of a matrix. Given that the underlying image distribution, $P_{\bm{S}}$ is unknown, it is impossible to calculate the exact $\mathcal{S}_1$ term. Thus, we estimate $\mathcal{S}_1$ by averaging over all the training set:
\begin{equation}
    \tilde{\mathcal{S}}_1 = \frac{1}{N_{tr}}\sum_{i=1}^{N_{tr}} \bm{s}_{1,i}\bm{s}_{1,i}^\dagger,
    \label{eq:covariance_est}
\end{equation}
where $N_{tr}$ and $\bm{s}_{1,i}$ denote the number of images in the training set and the complex vector $\bm{s}_1$ corresponding to the $i$-th image, respectively.

Finally, the optimization problem can be expressed as:
\begin{equation}
    \min_{\bm{F}_1} \|\bm{W}_1 - \bm{H}_1 \bm{F}_1\|^2_F + \lambda_1 \text{tr}(\tilde{\mathcal{S}}_1\bm{F}_1^H\bm{F}_1),
    \label{eq:optim_formulate}
\end{equation}
where $\lambda_1$ balances the classification accuracy and the transmit power consumption. We note that the naive solution, $\bm{F}_1 = \bm{H}^{-\dagger}_1 \bm{W}_1$ can be treated as a special case of \eqref{eq:optim_formulate} with $\lambda_1 = 0$.
It is easy to show that the optimization problem is convex which can be solved via gradient descent. For a given $\bm{H}_1$, the gradient is calculated and $\bm{F}_1$ is updated with a step size, $\eta$:
\begin{align}
    \nabla \bm{F}_1 &= -2\bm{H}_1^\dagger \bm{W}_1 + 2\bm{H}_1^\dagger \bm{H}_1 \bm{F}_1 + 2\lambda_1 \bm{F}_1 \tilde{\mathcal{S}_1}, \notag \\
    \bm{F}_1 &= \bm{F}_1 - \eta \nabla \bm{F}_1.
    \label{eq:gd_F}
\end{align}
The optimization process terminates when the deviation of the objective function in \eqref{eq:power_expect}, denoted as $G$ in two consecutive steps is smaller than $\epsilon$. The overall optimization process is summarized in Algorithm \ref{alg:calculate_Fi}. We calculate the precoding matrix $\bm{F}_i$ for each hop according to different statistics $\tilde{\mathcal{S}}_i$ and channel realizations, $\bm{H}_i$.  The performance of the optimization algorithm is evaluated in terms of the classification accuracy and the average transmit power $P_{avg}^t$ defined in \eqref{eq:P_avg_t}.

\subsection{Multiple Transmission Strategy}
We then consider the scenario where the relay nodes have limited number of antennas, denoted as $L < M$. This implies that the dimension of $\bm{s}_i$ needs to be reduced leading to degraded classification performance. In this subsection,  we will show by transmitting the signal $\lceil M/L \rceil$ times, the system with $L$ antennas is capable to support $M$-dimensional $\bm{s}_i$. We assume $M$ is a multiple of $L$ for simplicity, i.e., $M = JL$.

In the considered scenario, take the source node as an example. After generating $\bm{s}_1$, the source node partitions it into $J$ blocks, denoted as $\bm{s}_1 = [\bm{s}_1^1, \ldots, \bm{s}_1^J]$, then for the $j$-th block, the signal $\bm{s}_1^j$ is precoded by $\bm{F}_1^j$. We assume the channel matrix, $\bm{H}_1$ keeps constant over the $J$ transmissions and the received signal in the $j$-th time slot at the first relay can be expressed as $\bm{y}_1^j = \bm{H}_1 \bm{s}_1^j + \bm{n}_1^j$. By stacking the received signal for all the time slots, we obtain:
\begin{equation}
    \bm{y}_1 = (\bm{I}_J \otimes \bm{H}_1) \text{diag}(\bm{F}_1^1, \cdots, \bm{F}_1^J) \bm{s}_1,
    \label{eq:y1_T}
\end{equation}
where $\otimes$ stands for the Kronecker product and $\text{diag}(\cdot)$ denotes a diagonal matrix with the matrices, $\{\bm{F}_1^1, \cdots, \bm{F}_1^J\}$ as its diagonal elements. 

To obtain the precoding matrices, we follow the same procedure discussed above. In the training phase, for each hop, $J$ neural network weights, $\bm{W}_1^j \in \mathbb{C}^{L \times L}$ are obtained via end-to-end training. Then, given channel realization, $\bm{H}_1$, we calculate $\bm{F}_1^j$ using \eqref{eq:optim_formulate}:
\begin{equation}
    \min_{\bm{F}_1^j} \|\bm{W}_1^j - \bm{H}_1 \bm{F}_1^j\|^2_F + \lambda_1 \text{tr}(\tilde{\mathcal{S}}_1^j(\bm{F}_1^j)^\dagger\bm{F}_1^j),
    \label{eq:optim_formulate_t}
\end{equation}
where $\tilde{\mathcal{S}}_1^j$ denotes the expectation of $\bm{s}_1^j (\bm{s}_1^j)^\dagger$.
In the considered scenario with $L$ antennas, there are $ML$ learnable parameters for each hop, which is smaller than that with $M$ antennas where $M^2$ parameters are adopted. As will be shown in the simulation part, the framework with $L$ antennas is outperformed by that with $M$ antennas.

==> SecIV.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}{{0.64\columnwidth}}
         \centering
         \includegraphics[width=\columnwidth]{figures/diff_options.eps}
         \caption{}
     \end{subfigure}
     \begin{subfigure}{{0.64\columnwidth}}
         \centering
         \includegraphics[width=\columnwidth]{figures/num_hops.eps}
         \caption{}
     \end{subfigure}
    %  \vspace{0.1cm}
     \begin{subfigure}{0.64\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figures/transmit_power.eps}
         \caption{}
     \end{subfigure}
  \caption{Classification performance of the proposed scheme: (a) The performance obtained by the PrototypeNet adopting different loss functions, equipped with different number of antennas $M$, e.t.c. (b) The performance of the PrototypeNet with different number of hops $N$. (c) Performance of the multi-hop MIMO network compared with a direct precoding baseline.}
\label{fig:final_simu}
\end{figure*}

In this section, we evaluate the classification accuracy and the power consumption, $P_{avg}^t$ and $P_{avg}^r$ of the proposed multi-hop MIMO network.
The images are chosen from the Fashion MNIST dataset consisting of a training set with 60000 images and a test set of 10000 image. Each of the $28\times 28$ greyscale image belongs to $K = 10$ classes. We consider the number of hops $N = 1, 2, 3$, the number of antennas $M = 49$ and the noise variance, $\sigma^2$ is fixed at $0.1$.  
To train the PrototypeNet, we adopt the Adam optimizer with a learning rate equals to $5\times 10^{-4}$. 
The number of epochs and the batch size are set to $200$ and $32$, respectively.




\subsection{Performance Evaluation}
We first compare the performance of the PrototypeNet trained using two different loss functions described in \eqref{eq:optim_W} and \eqref{eq:optim_z}. In this simulation, the PrototypeNet corresponding to different loss functions are trained with different $\lambda$ values and we consider $N = 2$ hop.  As shown in Fig. \ref{fig:final_simu} (a), for a fixed $P^r_{avg}$ value, the PrototypeNet trained using the second loss function, i.e., $\mathcal{L}_2$ strictly outperform that using $\mathcal{L}_1$ which illustrates that it is more effective to directly minimize $P^r_{avg}$. Thus, in the rest of the paper, all the PrototypeNet are trained using $\mathcal{L}_2$. We also evaluate an alternative solution where the PrototypeNet is trained without noise yet tested with noise whose performance is shown in the dashed line. A significant performance degradation is observed showing that the weights trained without noise is fragile. 

The effectiveness of the multiple transmission strategy illustrated in Section \ref{sec:III} is also evaluated in Fig. \ref{fig:final_simu} (a). In this simulation, the multiple transmission scheme adopts $M = 7, J = 7$ and is compared with the single transmission scheme with $M = 7$. As can be seen, having multiple transmission leads to superior power-accuracy performance. However, it is outperformed by the $M = 49$ case as it has less number of learnable parameters for each hop. 
%We also consider evaluating the performance of the wireless network where the precoder matrices, $\bm{F}_i$ are obtained by solving the optimization problem in \eqref{eq:optim_formulate}. In particular, we consider $\lambda_1 = \{0, 0.1\}$ which correspond to the dashed lines in the same figure. As can be seen, when $\lambda_1 = 0$, $\bm{H}_i\bm{F}_i$ is exactly the neural network weight $\bm{W}_i$, thus it coincides with the curve of the PrototypeNet. The dashed line corresponding to $\lambda_1 = 0.1$ is inferior to that of the PrototypeNet as its aims to minimize the transmit power.

We then consider the performance obtained by different number of hops, $N$. In this simulation, we consider $N = 1, 2, 3$ and for each $N$, different PrototypeNet with different $\lambda$ values are trained. The power-accuracy performance with respect to different $N$ is shown in Fig. \ref{fig:final_simu} (b). The dashed lines represent the accuracy upper bound achieved by the PrototypeNet without noise. As can be seen, when $N$ is small, the accuracy upper bound is lower. This aligns with the intuition that, for a small $N$, we have less number of FC layers and the performance is limited due to the shallow neural networks. When the number of hops increases, the accuracy upper bound improves. 
We also observe that under a low $P^r_{avg}$, the PrototypeNet with a larger $N$ is outperformed by that with a small $N$. This can be understood that when $N$ becomes larger, the noise accumulates over the hops leading to less satisfactory results. It can be seen that when $P^r_{avg}$ grows, the accuracy of the PrototypeNet approaches its upper bound.

Finally, we outline the effectiveness of the proposed scheme by comparing with a baseline which is detailed as follows. In particular, for the $i$-th hop, the channel realization, $\bm{H}_i$ can be expressed using singular value decomposition (SVD): $\bm{H}_i = \bm{U}_i \bm{\Sigma}_i \bm{V}_i^\dagger$.
The transmitter ($\mathrm{R}_{i-1}$) precodes $\bm{s}_i$ using $\bm{V}_i$ and transmits it over the MIMO channel.  The $i$-th relay $\mathrm{R}_{i}$ combines the received signal $\bm{y}_i$ using $\bm{U}_i^\dagger$ and applies MMSE equalization to   generate an estimate of $\bm{s}_i$:
\begin{equation}
    \tilde{\bm{s}}_i = (\bm{\Sigma}_i^\dagger \bm{\Sigma}_i + \sigma^2 \bm{I}_M)^{-1}\bm{\Sigma}_i^\dagger \bm{U}_i^\dagger \bm{y}_i.
\end{equation}
The $\tilde{\bm{s}}_i$ is then power normalized and precoded to be transmitted over the $(i+1)$-th hop. Finally, the destination node estimates $\tilde{\bm{s}}_N$ which is fed to $f_c(\cdot)$ and the softmax function to generate the classification output.

We compare the proposed scheme with the baseline illustrated above. In this simulation, the average transmit power, $P_{avg}^t$ is considered and the number of hops $N$ equals to 2.  $\lambda_1$ are set to $0$ and $0.1$ for the proposed scheme.  As shown in Fig. \ref{fig:final_simu} (c), we can observe that when $P^t_{avg}$ increases, the proposed scheme outperforms the baseline adopting a direct precoding approach. It is also observed that superior performance is obtained with $\lambda_1 = 0.1$. This is because the randomly generated MIMO channel, $\bm{H}_i$ has a large probability to be ill-conditioned leading to large  $P^t_{avg}$ value which has been analyzed in Section \ref{sec:III}. The two dashed lines in the figure represent the results obtained via noiseless PrototypeNet with $N = 0, 2$ FC layers and they serve as the upper bound of the direct precoding and the proposed scheme, respectively.
We outline that the proposed scheme with $\lambda_1 = 0.1$ outperforms the baseline when $P^t_{avg} > 5$ dB which shows the effectiveness of the PrototypeNet and the optimization procedure demonstrated in Algorithm \ref{alg:calculate_Fi}.
